Domain Generalization by Mutual-Information Regularization with Pre-trained Models

Domain generalization (DG) aims to learn a generalized model to an unseen target domain using only limited source domains. Previous attempts to DG fail to learn domain-invariant representations only from the source domains due to the significant domain shifts between training and test domains. Instead, we re-formulate the DG objective using mutual information with the oracle model, a model generalized to any possible domain. We derive a tractable variational lower bound via approximating the oracle model by a pre-trained model, called Mutual Information Regularization with Oracle (MIRO). Our extensive experiments show that MIRO significantly improves the out-of-distribution performance. Furthermore, our scaling experiments show that the larger the scale of the pre-trained model, the greater the performance improvement of MIRO. Source code is available at https://github.com/kakaobrain/miro.

==> figures/__acc_by_target.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/acc_by_target_fig.pdf}
    \caption{\textbf{Performance changes for tuned $\lambda$ of various models.} X-axis indicates pretraining methods; \textit{IN} indicates ImageNet ERM, \textit{BT} and \textit{MoCo} indicate Barlow Twins \cite{zbontar2021barlowtwins} and MoCo v3 \cite{chen2021mocov3} self-supervised pretraining, \textit{CLIP} indicates contrastive language-image pretraining (CLIP) \cite{radford2021clip} where $\dagger$ indicates ViT-Base architecture, and \textit{SWAG} indicates SWAG weakly supervised pretraining method with RegNetY-16GF architecture. The methods not specifying an architecture use ResNet-50 as default.}
    \label{fig:acc_by_target}
\end{figure}

==> figures/camelyon_examples.tex <==
\begin{figure}[tb]
\begin{center}
\setlength{\tabcolsep}{0pt}
\newcommand\figwidth{.15}
\newcommand\rf{-0.4}
\newcommand\rs{-0.45}
\renewcommand{\arraystretch}{1.3}

\begin{tabular*}{0.8\textwidth}{c @{\extracolsep{\fill}} ccccc}
    \rotatebox[origin=c]{90}{Normal}
    &
    \raisebox{\rf\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T0_H0.png}}
    &
    \raisebox{\rf\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T0_H1.png}}
    &
    \raisebox{\rf\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T0_H2.png}}
    &
    \raisebox{\rf\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T0_H3.png}}
    &
    \raisebox{\rf\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T0_H4.png}}
\\
    \rotatebox[origin=c]{90}{Tumor}
    &
    \raisebox{\rs\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T1_H0.png}}
    &
    \raisebox{\rs\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T1_H1.png}}
    &
    \raisebox{\rs\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T1_H2.png}}
    &
    \raisebox{\rs\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T1_H3.png}}
    &
    \raisebox{\rs\height}{\includegraphics[width=\figwidth\textwidth]{figures/camelyon_images/T1_H4.png}}
\\
    &
    {\small Hospital 1}
    &
    {\small Hospital 2}
    &
    {\small Hospital 3}
    &
    {\small Hospital 4}
    &
    {\small Hospital 5}
\end{tabular*}
%
\end{center}
\caption{\small \textbf{Example images of \data{Camelyon17}.} Distribution shifts between hospitals are caused by the way to acquire and process the tissue slide images.
}
\label{fig:camelyon_examples}
\end{figure}

==> figures/tsne.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.3\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne/PACS_PT.pdf}
        \caption{\small Pre-trained}
        \label{fig:tsne-pretrained}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne/PACS_ERM.pdf}
        \caption{\small ERM}
        \label{fig:tsne-erm}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.3\linewidth}
        \includegraphics[width=\linewidth]{figures/tsne/PACS_MIRO.pdf}
        \caption{\small MIRO}
        \label{fig:tsne-miro}
    \end{subfigure}
    % \hfill

    \caption{\small \textbf{t-SNE visualization of features in \pacs{}.} Different color indicates different training domain.}
    \label{fig:tsne}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\columnwidth]{figures/mi_all.pdf}
%     \caption{\textbf{Mutual information with oracle model.} \textit{Random} is randomly initialized model, \textit{Scratch} is trained by ERM from \textit{Random}, and \textit{Pretrained} is initialized by pretrained model without training. \textit{ERM} and \textit{SIL} is initialized by pretrained model and trained by each method. $\dagger$ indicates RegNetY-16GF pretrained by SWAG is used and ResNet-50 pretrained in ImageNet is used for the others.}
%     \label{fig:mi}
% \end{figure}




